Kalman Filter-based Head Motion Prediction for Cloud-based Mixed Reality

Volumetric video allows viewers to experience highly-realistic 3D content with six degrees of freedom in mixed reality (MR) environments. Rendering complex volumetric videos can require a prohibitively high amount of computational power for mobile devices. A promising technique to reduce the computational burden on mobile devices is to perform the rendering at a cloud server. However, cloud-based rendering systems suffer from an increased interaction (motion-to-photon) latency that may cause registration errors in MR environments. One way of reducing the effective latency is to predict the viewer's head pose and render the corresponding view from the volumetric video in advance. In this paper, we design a Kalman filter for head motion prediction in our cloud-based volumetric video streaming system. We analyze the performance of our approach using recorded head motion traces and compare its performance to an autoregression model for different prediction intervals (look-ahead times). Our results show that the Kalman filter can predict head orientations 0.5 degrees more accurately than the autoregression model for a look-ahead time of 60 ms.

==> background.tex <==
\section{Background}
\label{sec:background}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.9\linewidth]{img/overview}
    \caption{Overview of the system components and interfaces.}
    \label{fig:overview}
\end{figure*}

In this section, we briefly review some of the works in the literature on volumetric video streaming, cloud rendering systems and head motion prediction techniques.
\subsection{Volumetric video streaming}
Volumetric video is typically created by capturing the scene from all directions using multiple synchronized cameras. Then, a dynamic 3D model (mesh or point cloud) is created from the captured views~\cite{schreer2019icip}. 
Some recent works present initial frameworks for streaming of volumetric videos. 
Qian et al.~\cite{qian2019} developed a proof-of-concept point cloud streaming system and introduced optimizations to reduce the \gls{m2p} latency.
Park et al.~\cite{park2019} designed an adaptive volumetric video streaming system that adapt the \gls{lod} of 3D tiles depending on the distance of the user. Furthermore, they introduced a greedy algorithm to allocate bits between different tiles across multiple objects for rate-utility optimization.
Van der Hooft et al.~\cite{van2019} proposed an adaptive streaming framework compliant to the recent point cloud compression standard MPEG V-PCC~\cite{schwarz2018}. They used their framework for HTTP adaptive streaming of scenes with multiple dynamic point cloud objects and presented a rate adaptation algorithm that considers the user's position and focus.
Petrangeli et al.~\cite{petrangeli2019} proposed a streaming framework for \gls{ar} applications that dynamically decides which virtual objects should be fetched from the server as well as their \glspl{lod}, depending on the proximity of the user and likelihood of the user to view the object. 
%Thus, they aimed to maximize the object's perceived visual quality. They carried out their experiments using an AR streaming prototype developed on an iOS device.

\subsection{Cloud rendering systems}
The concept of remote rendering was first put forward to facilitate the processing of 3D graphics rendering when PCs did not have sufficient computational power for intensive graphics tasks. A detailed survey of interactive remote rendering systems in the literature is presented in ~\cite{shi2015}. 
%In recent years, with the increasing network speeds and rise of cloud computing, the concept has re-emerged in the context of cloud-based streaming of computer games as well as \ang{360} and volumetric videos. 
Shi et al.~\cite{shi2019} proposed a \gls{mec} system to stream \gls{ar} scenes containing only the user's \gls{fov} and a latency-adaptive margin around the \gls{fov}. They evaluate the performance of their prototype on a \gls{mec} node connected to a 4G (LTE) testbed.
Mangiante et al.~\cite{mangiante2017} proposed an edge computing framework that performs \gls{fov} rendering of \ang{360} videos. Their system aims to optimize the required bandwidth as well as reduce the processing requirements and battery utilization.

Cloud rendering has also started to receive increasing interest from the industry, especially for cloud gaming services. Nvidia CloudXR~\cite{nvidia2019} provides an SDK to run computationally intensive \gls{xr} applications on Nvidia cloud servers to deliver advanced graphics performances to thin clients. Google Stadia~\cite{google2019}, a cloud gaming service operated by Google, has already been launched in November 2019. Microsoft has also started trials of its Xbox game streaming service Project xCloud~\cite{microsoft2019} and is expected to launch its service in 2020.

\subsection{Head motion prediction techniques}
\label{sec:bg_prediction}
Several sensor-based methods have been proposed in the literature that attempt to predict the user's future viewport for optimized streaming of \ang{360}-videos.
%Those can be classified into three main categories depending on the kind of information they rely on: i) sensor data, ii) content analysis, iii) data-driven (statistical). 
Those can be divided into two categories. Works such as~\cite{bao2016, bao2017, sanchez2019, aykut2018, oculus16} were specifically designed for \gls{vr} applications and use the sensor data from \glspl{hmd} whereas the works in~\cite{barniv2005, koirala2015, bai2011} attempt to infer user motion based on some physiological data such as \gls{eeg} and \gls{emg} signals.
Bao et al.~\cite{bao2016} collected head orientation data and exploited the correlations in different dimensions to predict the head motion using regression techniques. Their findings indicate that \glspl{lat} of \SIrange{100}{500}{ms} is a feasible range for sufficient prediction accuracy.
Sanchez et al.~\cite{sanchez2019} analyzed the effect of \gls{m2p} latency on a tile-based streaming system and proposed an angular acceleration-based prediction method to mitigate the impact on the observed fidelity. 
Barniv et al.~\cite{barniv2005} used the myoelectric signals obtained from \gls{emg} devices to predict the impending head motion. They trained a neural network to map \gls{emg} signals to trajectory outputs and experimented with combining \gls{emg} output with inertial data. Their findings indicate that a \glspl{lat} of \SIrange{30}{70}{ms} are achievable with low error rates. 
Bai et al.~\cite{bai2011} attempted to utilize \gls{eeg} signals to anticipate the impending head motion. They reported an average \gls{lat} of \SI{0.62 \pm 0.25}{\s}; however, they also noted that some predictions occur without subsequent head movements (false positives).
% Content-based methods such as~\cite{deabreu2017, ozcinar2018, ozcinar2019} employ saliency maps which are estimated using \gls{vp} trajectories and visual attention models. De Abreu et al.~\cite{deabreu2017} collected the center trajectories of \glspl{vp} from several users and proposed a method to transform the gathered data into saliency maps. Ozcinar et al.~\cite{ozcinar2018} created a new visual attention user dataset for omnidirectional videos and analyzed the prediction performance of the state-of-the-art visual attention models. In their follow-up work~\cite{ozcinar2019}, they introduced an adaptive \ang{360} video streaming framework that optimizes the DASH representations of \ang{360} content considering their visual attention maps. Fan et al.~\cite{fan2017} employed both sensor- and content-related features to train two neural networks which accurately predict user fixations. 

% Data-driven methods such as~\cite{petrangeli2018, liu2017, xu2018} collect user statistics and try to predict the future user position based on statistical models. Petrangeli et al.~\cite{petrangeli2018} modeled the \gls{vp} evolution of users over time as a trajectory and clustered the trajectories with similar viewing behaviors For each cluster, they created different models to predict the future \gls{vp} at run-time. Liu et al.~\cite{liu2017} combined different kinds of data; namely the viewing statistics of a video across users, viewing behaviors of multiple videos by a single user and other contextual cues to prefetch future chunks of content based on their predictions. Xu et al.~\cite{xu2018} leveraged the probability distribution of the user's orientation and designed an algorithm that prefetches segments by maximizing the expected quality.

Most of the previous works target \gls{3dof} \gls{vr} applications and thus focus on prediction of only the head orientation in order to optimize the streaming \ang{360} videos. However, little work has been done so far on prediction of \gls{6dof} movement for advanced \gls{ar} and \gls{vr} applications. In Sec.~\ref{sec:prediction}, we present an initial statistical model for \gls{6dof} prediction and discuss our findings. 


